Manipulating OpenFlow Link Discovery Packet Forwarding for Topology Poisoning

Software-defined networking (SDN) is a centralized, dynamic, and programmable network management technology that enables flexible traffic control and scalability. SDN facilitates network administration through a centralized view of the underlying physical topology; tampering with this topology view can result in catastrophic damage to network management and security. To underscore this issue, we introduce Marionette, a new topology poisoning technique that manipulates OpenFlow link discovery packet forwarding to alter topology information. Our approach exposes an overlooked yet widespread attack vector, distinguishing itself from traditional link fabrication attacks that tamper, spoof, or relay discovery packets at the data plane. Unlike localized attacks observed in existing methods, our technique introduces a globalized topology poisoning attack that leverages control privileges. Marionette implements a reinforcement learning algorithm to compute a poisoned topology target, and injects flow entries to achieve a long-lived stealthy attack. Our evaluation shows that Marionette successfully attacks five open-source controllers and nine OpenFlow-based discovery protocols. Marionette overcomes the state-of-the-art topology poisoning defenses, showcasing a new class of topology poisoning that initiates on the control plane. This security vulnerability was ethically disclosed to OpenDaylight, and CVE-2024-37018 has been assigned.

==> attack_single_controller.tex <==
\vspace{-5pt}
\subsection{Attacking SDN controllers}\label{sec:eval_controller}

\input{tables/controllers}

We evaluate 5 popular open-source SDN controllers (Table~\ref{table_controllers}) using the illustrative example introduced in \S\ref{sec:approach} assuming a topology poisoning attack initiated by a malicious application. We deploy mininet-v2.2.2, Floodlight-v1.2, OpenDaylight-v0.15.3, ONOS-2.2.0, Ryu-v4.34, and pox-v\_eel on six connected VMs with Linux systems on the CyberVAN testbed~\cite{chadha2016cybervan}. 

%Topology poisoning attacks on a single controller originate from malicious SDN applications.

Among the five controllers, only OpenDaylight and Floodlight have implemented security enhancements by introducing hash checks on LLDP packets~\cite{wazirali2021sdn}. However, the hash check mechanism does not defend against \projname{} as our technique does not tamper with LLDP packets but modifies the path taken by the LLDP packets. Indeed, we achieved precise topology poisoning 
%resulting in the deceptive topology shown in Figure \ref{fig:fab_topo} 
on all controllers. %In Figure \ref{fig:topo_pois_controllers}, we present the results of the attack on RYU, Floodlight, and ONOS (The colored marks in Figure \ref{fig:fab_topo_onos} correspond to the colored links in Figure \ref{fig:fab_topo}). 

Interestingly, while Ryu and ONOS lack security enhancements in discovering the topology, they present additional challenges in launching a successful attack. Ryu sets its flow entries for forwarding LLDP packets back to the Ryu controller with the highest priority in the flow table.  As a result, \projname{} must lower the priority of the entries set by the Ryu controller before initiating the attack.  
%\trent{I don't get this one.}\tpt{I tried editing this.. any better?}

ONOS employs per-logical-plane fingerprints encoded on the \kw{ether-src} field, resulting in a unified value of \kw{ether-src} per cluster. As a result, VLAN-based poisonous flow entry matching [\kw{ether-src}, \kw{in-port}] is mandatory to identify the source of discovery packets for all three deceptive links. Details are described in Section \ref{sec:vlanentries}. \update{To conclude, \projname{} can attack all 5 open-source controllers. }
%For each link fabrication described in \S\ref{sec:approach}, we utilize \kw{ether-src} combined with \kw{in-port} as the match criteria for the poisonous flow entry and configure it on the first-hop switch to push the VLAN tag and forward. Consequently, an additional poisonous flow entry with the match on \kw{vlan\_id} and actions of (\kw{pop-vlan}, \kw{to\_controller}) is required at the destination node. %As a result, ONOS requires 14 poisonous flow entries whereas the other controllers need only 8 to successfully execute the attack.



\inlinedsection{Discussion}
Discovery packet flow entries are static and specifically serve the control plane. As a result, they should not be changed or overridden easily by arbitrary controllers. Unfortunately, there is currently no access control mechanism for flow entry enforcement implemented in any of the SDN controllers examined.


==> background_SDN.tex <==
\subsection{OpenFlow and OpenFlow Link Discovery}


\update{OpenFlow~\cite{openflow} is a standard SDN protocol that allows a controller to gather information and instruct switches on how to route incoming packets by sending them flow entries\footnote{The flow entry has a \emph{match} field and a set of \emph{actions} to apply to the matched packets. Entry types for matching include source/destination MAC and IP addresses, VLAN ID, input port, etc. Instructions associated with each entry may contain actions instructing packet forwarding, packet modification, group table processing, etc.}. When a packet arrives at a switch, the switch checks its flow table to determine whether there is a matching flow entry to determine where to forward the packet. If yes, the switch forwards the packet accordingly. Otherwise, it encapsulates the packet in a \kw{packet-in} message and sends it to the controller due to a table-miss flow entry. A table-miss flow entry is the default flow entry instructing the unmatched packet to be sent to the controller. Once the controller determines the route, it sends the packet back to the switch encapsulated in a \kw{packet-out} message and installs necessary flow entry\footnote{When the controller fails to determine an output at the current switch (because the destination host is unknown or the switch is not on the computed route), the controller sends the packet back to the switch and instructs it to flood this packet through all its ports.} in the switch using \kw{flow-mod} messages. The controller repeats this process until the packet arrives at its destination. This process is called \emph{reactive forwarding}. The controller can also configure flow entries beforehand spontaneously, which is called \emph{proactive forwarding}.}
  

To maintain correct centralized control of modern, dynamically changing networks, controllers (re-)discover the network topology frequently (e.g., commonly every 100 ms), via the OpenFlow Discovery Protocol (OFDP).
In Figure~\ref{fig:ofdp}, we illustrate a single instance of OFDP discovering a unidirectional link from \switch{A} to \switch{B}. The OFDP process is initiated in step \ding{192} when the controller sends a \kw{packet-out} message encapsulating an LLDP packet, which we denoted as $LLDP_{A2}$, to switch~\switch{A} and instructs \switch{A} to forward the LLDP to port 2. 
In step \ding{193}, switch~\switch{A} receives the \kw{packet-out} message, decapsulates the OpenFlow header, and sends the $LLDP_{A2}$ packet to port 2; switch~\switch{B} receives the $LLDP_{A2}$ packet sent from (\switch{A}, Port: 2) (\ding{194}).
%. \trent{At port 1?} 
The LLDP packet matches the pre-configured table-miss /LLDP flow entry\footnote{match: ``ether-type:0x88cc", where ``0x88cc" is LLDP packet type} in switch~\switch{B} which instructs the switch to send it to the controller using a \kw{packet-in} message. Finally, in step \ding{195}, the controller receives the \kw{packet-in} message. It learns that the $LLDP_{A2}$ packet was sent from (\switch{A}, Port:2) by checking the $LLDP_{A2}$ payload, and received by (\switch{B}, Port:1) 
%\trent{B port 1?} 
by checking the \kw{packet-in} payload. The controller writes a unidirectional link (\switch{A}, Port:2) $\rightarrow$ (\switch{B}, Port:1) to its data store. Hereafter, we use the notation $A2\rightarrow1B$ for simplicity. 

There have been many modifications to OFDP to improve performance. Table~\ref{table_protocols} (\S\ref{sec:eval_protocol}) lists all wire SDN discovery protocols~\cite{wazirali2021sdn} and analyzes our attack against each protocol.

\begin{figure}[t]
  \centering
  \begin{minipage}[b]{0.23\textwidth}
    \includegraphics[width=\textwidth]{figs/OFDP.png}    
    \caption{OFDP illustration}
    \label{fig:ofdp}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.22\textwidth}
    \includegraphics[width=\textwidth]{figs/threat_model.png}    
    \caption{Threat Model}
    \label{fig:threat_model}
  \end{minipage} 
  \vspace{-10pt}
\end{figure}


==> gap-patching_computation.tex <==

\subsection{Gap Patching Computation and Setup}\label{sec:gap_patching}

Once the topology has been poisoned, the routes calculated by the benign leader controller based on the deceptive topology may contain gaps as described in \S\ref{sec:gappatchentries}. %because the leader controller is not aware of the full path that comprises a fabricated link. 
We address this proactively and reactively. For proactive patching, we set the gap-patching and poisonous flow entries together because we can predict the new routes for existing flows. In reactive forwarding mode, \update{the controller instructs the switch to flood this unexpected packet~\footnote{When a packet is forwarded to the controller by a switch, but the switch's position contradicts the packet's routing path based on the recent topology, we designate it as an unexpected packet to the switch.} with \kw{packet-out} message to all its ports.} This behavior provides \projname{} with ample time to patch the gaps. In this context, the latency performance of the gap-patching model primarily affects stealthiness rather than persistence. Reducing the number of unexpected packets sent to benign controllers results in a lower level of suspicion. The details of the gap-patching algorithm are in Appendix \ref{sec:appendix_gap_patching}.



==> poison_computation.tex <==
\subsection{Poison Computation and Setup}\label{sec:pois_link}

Once the RL workflow creates a poisonous topology, \projname{} generates and installs the poisonous flow entries to realize the deceptive topology. In \S\ref{sec:approach}, we introduced a topology poisoning attack using poisonous flow entries and provided examples of simple link poisoning. However, in large network scenarios, the setup of poisonous flow entries can become complex due to the sheer number of possible links that can be manipulated with possible intermediate nodes along the path. To scale our approach, we designed a general algorithm for computing the necessary poisonous flow entries for each hop, taking into account the network topology, switch nodes, and a deceptive link as input. The algorithm described in Algorithm~\ref{alg:pois_link} (Appendix \ref{sec:appendix_pois_flow_entry}) implements Rule \ref{rule_link}, focusing on how to ensure that the discovery packet sent from $(A, Port:x)$ is received at $(B, Port:y)$. The details are in Appendix \ref{sec:appendix_pois_flow_entry}.

==> poisonous_flow_entry_details.tex <==
\section{Poisonous Flow Entry Computation}\label{sec:appendix_pois_flow_entry}
\begin{figure}[t]
     \centering
     \includegraphics[width=0.5\textwidth]{figs/alg_pois_v.png}
     %\vspace{-20pt}
    \caption{Algorithm of Link Poisoning}
        \label{fig:alg_pois}
        %\vspace{-0.3\baselineskip}
\end{figure}

Figure \ref{fig:alg_pois} shows a VLAN-based link poisoning algorithm that uses the \kw{ether-src}-distinguishable VLAN poisonous flow entries described in Section \ref{sec:approach}. Information about the link is collected in Lines 1--4. There may be multiple paths that can be used to build $Ax\rightarrow yB$, but the shortest path between $A$ and $B$ is not necessarily the best. Lines 5--11 determine which path will minimize the number of required poisonous flow entries. 


While we use Dijkstra's shortest path routing algorithm to compute the poisoning path, additional poisonous flow entry setups may be required depending on the target deceptive link. In certain situations, it is necessary to forward the packet back to its received port. To guarantee that we can fabricate links that terminate on the proper ports of the switches, there are two methods to create poisonous paths. The first is a direct method that results in a \textit{no-loop} path.  In circumstances in which the direct method cannot terminate the poisonous link on the correct port, we must use an indirect method that results in a \textit{loopback} poisonous path.  Suppose the deceptive link is $A1\rightarrow 2B$ shown in red in Figure \ref{fig:sele_rou}. The discovery packet is initiated by the controller and sent to $A$ within a \kw{packet-out} message. $A$ sends the discovery packet to the first hop $C$ (which is $src$ in Line 3). 
This process cannot be manipulated by \projname{} because the framework does not tamper with the \kw{packet-out} message; therefore, $C$ is the source of our shortest path calculation to find a path from $A1$ to $2B$.  However, Dijkstra's algorithm is not port number sensitive. As a result, it returns a solution of the shortest path ($C\rightarrow B$) with length 1, but as shown, the direct path does not terminate on $(B, Port:2)$. In this case we must resort to the indirect method to find the {loopback} path.   
To accomplish this, the discovery packet must be sent out through $(B, Port:2)$ and have $(D, Port:2)$ send it back so it can be received at $(B, Port:2)$ as shown in Figure~\ref{fig:loopback}.
We need the loopback in certain cases because if we are targeting $(B, Port:2)$ the LLDP packet must be received on a port from a link \textit{outside} the switch to be checked against the switch's flow table, and then passed to the controller. 

\begin{figure}[t]
%\vspace{-1\baselineskip}
\centering
\subfigure[Loopback Method]{\label{fig:loopback} \includegraphics[width=0.2\textwidth]{figs/loopback.png}}% The "%" masks the line break.
\hfill
\subfigure[No-loop Method]{\label{fig:no_loop} \includegraphics[width=0.22\textwidth]{figs/no-loop.png}}%
\hfill
%\vspace{-1.5\baselineskip}
\caption{Path selection of Loopback and No-loop methods}
\label{fig:sele_rou}
%\vspace{-0.3\baselineskip}
\end{figure}

While the loopback method can %The Loopback method in Figure \ref{fig:loopback} can 
create deceptive links successfully, it may require more flow entries than needed.  In the example, three flow entries are configured on three switches ($C$, $B$, $D$). By contrast, the no-loop method shown in Figure~\ref{fig:no_loop} only requires two entries on $C$ and $D$. When this is the case, the algorithm chooses the no-loop method (lines 5--7); when it is not, it chooses the loopback method (lines 8--11). 

The poisonous flow entries computed in Lines 12--41 forward the discovery packet along the poisoning path. There are four types of flow entries. The $E_{VStart}$, $E_{VEnd}$, and $E_{VBody}$ flow entries are for building the VLAN poisonous paths (the green paths in Figure~\ref{fig:sele_rou}) as described in \S\ref{sec:vlanentries}. $E_{VStart}$ adds a VLAN tag to an LLDP packet and sends it out, $E_{VEnd}$ matches the VLAN tag, removes the tag and forwards the original packet, and $E_{VBody}$ simply matches the tag and forwards the packet. $E_{hop}$ (lines 20--21) is the flow entry for a single hop when the path is too short to build a VLAN tunnel and only a single hop is needed.
% as in Figure~\ref{fig:fab_link}. 
%
In lines 12--17, we compose the matches and actions for $E_{hop}$, $E_{VStart}$, $E_{VEnd}$, and $E_{VBody}$ based on the vanilla and VLAN poisonous flow entry design discussed in \S\ref{sec:approach}. In lines 18--41, we relay the discovery packet as appropriate to either set up a VLAN tunnel with or without loopback or relay the packet a single hop if that is sufficient to build the deceptive link. 

There are two critical points when composing the VLAN flow entries. First, the loopback can happen at both the beginning (lines 23--26) (called head loopback) and the end (lines 33--41) (called tail loopback) of the VLAN tunnel.  Second, nodes that act as both the initiator of a tail loopback, and the beginning node for a VLAN tunnel must be carefully crafted to avoid flow entry conflict (lines 36--39). In such instances, the same discovery packets will be received twice at the node, but require different actions; therefore, we need to distinguish at what stage of the forwarding sequence the packet is in by matching against the \kw{in-port} and \kw{ether-src} fields.

\iffalse
\section{Poisonous Flow Entry}
The basic idea of the remaining parts of the algorithm is building the VLAN start, VLAN body, and VLAN end with $E_{VStart}$, $E_{VBody}$, and $E_{VEnd}$ flow entries\tpt{Where did these entries appear from? We need context. This subsection is heavy in technical content and it's hard to follow for a non-SDNer}. Normally, the VLAN starts at $sub\_src$ and ends at $sub\_dst$ so $B$ will receive the original packet. When VLAN is mandatory to identify the source of the discovery packet and the poisoning path is only one hop length as the case in Fig. \ref{fig:fab_topo}, the VLAN ends at $B$ with actions of (pop-vlan, to\_controller).
In Lines 12-17, necessary matches and actions are defined for VLAN-built usage. In detail:
\begin{itemize}
    \item $match\_simple$: Match on $ether-src$. When the $ether-src$ is unavailable to identify the discovery packet source due to being unified or randomized, use $[ether-dst, in-port]$ as discussed in Sec. \ref{sec:approach}.
    \item $match\_inport$: Match on $ether-src$ and $in-port$ to prevent the reflected discovery packet from matching on it repeatedly causing an endless loop on the Loopback part.
    \item $match\_Vid$: Match on $VLAN\_ID$.
    \item $actions\_simple(out\_port\_num)$: Output packet to $out\_port\_num$.
    \item $actions\_pushV(out\_port\_num)$: Push a VLAN ID on a packet and output the packet to $out\_port\_num$.
    \item $actions\_popV(out\_port\_num)$: Pop a VLAN ID from a packet and output the packet to $out\_port\_num$.
\end{itemize}

Lines 18-32 are the No-loop part with or without the tail Loopback part \tpt{first use of tail loopback part}. The $out\_port\_num$ is extracted from the link information to support corresponding hops. Lines 20-21 are for the single hop case where only ($match\_simple, actions\_simple(out\_port\_num)$) is necessary. Otherwise, lines 22-26 are the VLAN start that has flow entries $E_{VStart}$ with ($match\_simple, actions\_pushV(out\_port\_num)$). Especially, the $out\_port\_num$ is $IN\_PORT$ which means a head Loopback when the next hop of the $sub\_src$ is $A$ in Lines 23-25. Lines 27-29 build the VLAN end using flow entries $E_{VEnd}$ with ($match\_Vid$, $actions\_popV(out\_port\_num)$) on the $sub\_dst$ if there is no tail Loopback part. Lines 30-31 are the VLAN body using flow entries $E_{VBody}$ with ($match\_Vid$, $actions\_simple(out\_port\_num)$).

Lines 33-41 are the Loopback part if required. When the length of the chosen path is more than 1, the Loopback part starts at VLAN body using $E_{VBody}$ on $B$ with ($match\_Vid$, $actions\_simple(y)$)(Lines 33-35). When the length of the chosen path is 1, the Loopback part start is the VLAN start which means the $sub\_src$ is the $B$. This case is only meaningful when $A$ and $B$ are directly connected but $Ax$ connects with $zB$ ($y \neq z$) in real topology because a real link can not be the input fake link. The $match\_inport$ with $actions\_simple(y)$ is needed to prevent the reflected VLAN-popped discovery packet from matching on it again(Lines 36-39). At last the Loopback end is the VLAN end for any cases, the flow entries $E_{VEnd}$ is on the $sub\_dst$ with ($match\_Vid$, $actions\_popV(IN\_PORT)$).
\fi


==> tables/related_attacks.tex <==
\begin{table*}[hbt!]
\caption{Related Threats and State-of-the-art Defences}\label{table:related_threat}
%\vspace{-0.8\baselineskip}
\begin{tabular}{p{1.4cm}p{3.8cm}p{1.28cm}p{4.7cm}|p{2.4cm}p{2cm}}
    \toprule
    \textbf{Attack Surface} & \textbf{Attack Methodology}  &
    \textbf{Impact} & \multicolumn{3}{p{6.8cm}}{\textbf{Defense}} \\
    \midrule
     Malicious Host(s)/ Switch     
     & \multirow{5}{3.9cm}{\attack{1} 
     \textbf{Link Fabrication:}
     Fabricate a deceptive link A1 -> B2 on the controller's view. \\
     
     Methods: 1. Relay LLDP packet from A1(switch A port 1) to B2 by: 
     \begin{enumerate}[leftmargin=1.4em]
         \item malicious hosts~\cite{hong2015poisoning,skowyra2018effective}
         \item malicious switch~\cite{alimohammadifar2018stealthy}  \\
         ("Match: ether-type: 0x88cc, inport:1 Action: 2"~\cite{al2022link})
     \end{enumerate}
     2. Fabricate LLDP packet with "src: A1" and send it to B2 by:
     \begin{enumerate}[leftmargin=1.4em]
        \setcounter{enumi}{2}
         \item malicious hosts~\cite{hong2015poisoning,skowyra2018effective}
         \item malicious switch~\cite{baidya2020link}
     \end{enumerate}}
      % & \multirow{5}{1.3cm}{Localized Persistent}
      & Localized Persistent
      & \multicolumn{3}{p{9.8cm}}{\defense{1} SPV: With benign controller assumption, it sends a probe to go through the target link. If the link is fabricated, the probe forwarding through A1 will be dropped or fed back to the controller by a switch port other than B2~\cite{alimohammadifar2018stealthy}.}\\
      \cmidrule{4-6}
      & &  & \multicolumn{3}{p{9.8cm}}{\defense{2} Latency-based Detection: A link is considered fabricated if its latency is greater than a threshold value~\cite{smyth2017detecting,huang2020towards,al2022link,gao2022defense}.}\\
      \cmidrule{4-6}
      & &  & \multicolumn{3}{p{9.8cm}}{\defense{3} Sphinx: With benign controller assumption, it builds the flow graph incrementally from Flow-mod OF-message, comparing it with actual flow routings using switch metadata. If a discrepancy is found, fabricating links are on the differing points~\cite{dhawan2015sphinx}.}\\
      \cmidrule{4-6}
      & &  & \multicolumn{3}{p{9.8cm}}{\defense{4} Port-based Detection: If an active port connects more than one link, either switch-host link or switch-switch link, one of the switch-switch links is fabricated~\cite{baidya2020link,dhawan2015sphinx}.}
     \\
     \cmidrule{4-6}
     & &  & \multicolumn{3}{p{9.8cm}}{\defense{5} TopoGuard(+): If an active port connects with both host and switch, the link connects switch is fabricated; Authenticating LLDP packets to prevent LLDP packet fabrication~\cite{hong2015poisoning,skowyra2018effective}.} \\
    \cmidrule{1-6}
    
    \multirow{3}{1.6cm}{Malicious Application/ Controller in Cluster} &  \multirow{2}{3.8cm}{\attack{2} \textbf{Wrong Information Sharing:} Malicious controller shares wrong (topology) information in the controller cluster to cause topology poisoning~\cite{khan2016topology, ropke2018preventing, maleh2023comprehensive}.} & Globalized Ephemeral & \defense{6} Dynamic Cluster: Leader controller is dynamically assigned~\cite{hu2018multi,zhang2018survey,tootoonchian2010hyperflow} and it periodically (e.g., every 100 milliseconds ~\cite{wazirali2021sdn})
    re-discovers the topology from the network independently~\cite{wazirali2021sdn,azzouni2017softdp,dhawan2015sphinx}. & \multirow{2}{2.5cm}{\defense{7} Monitoring-based Detection: Defenses~\cite{zhou2018sdn,ujcich2018cross,ujcich2021causal,ropke2018preventing} audit the controller's or applications' behavior to detect anomalies by backup controller, information flow model, root causes, or comparison with real network state.}& \multirow{2}{2.2cm}{\defense{8} Voting-based Defense: Fleet~\cite{matsumoto2014fleet},  \textsc{topotrust}~\cite{adjou2022topotrust}, and Mcad-SA\cite{qi2016intensive} depend on the majority to vote out a malicious controller based on odd behaviors around reactive forwarding or spoofing. }\\
    
    \cmidrule{2-4}
    & \multirow{3}{3.8cm}{\attack{3} \textbf{Malicious Routing:} Insert malicious flow entries to conflict with existing traffic-routing flow entries to detriment flow routings, network policy, or other applications~\cite{khurshid2012veriflow, porras2012security, al2010flowchecker,kazemian2013real, ujcich2018cross, habib2022mitigating}.}& Globalized Persistent & \defense{9} Flow Rule Checker: Veriflow~\cite{khurshid2012veriflow}, FlowChecker~\cite{al2010flowchecker}, Netplumber~\cite{kazemian2013real}, Eirene~\cite{habib2022mitigating}, and FortNOX~\cite{porras2012security} build the flow graph/logic with header information (e.g.src/dst IPs/ports) of flow entries to detect flow rule conflicts and policy violations. & &\\
    % \cmidrule{4-6}
    
    
    \cmidrule{2-6} 
    & \textbf{\projname{}}: Insert poisonous flow entries to bypass table-miss/LLDP flow entries to poison the topology. & Globalized Persistent & \multicolumn{3}{p{9.8cm}}{\textbf{No existing defense against \projname{}} because: existing defenses have overlooked the vulnerability where regular flow entries conflict with table-miss and LLDP flow entries (which is called priority-bypassing attack more specifically) to manipulate link discovery results, as detailed in Table \ref{table:features}.
    }\\
    %It cannot be detected unless \defense{7} combines with \defense{1}, or \defense{7} knows the switch port MAC addresses, and realizing flow entries matching those MAC addresses can influence topology discovery. }\\
    \bottomrule
\end{tabular}
\vspace{-0.8\baselineskip}
\end{table*}






%~\cite{kreutz2014software}Cited by 6209: " A compromised critical computer, directly connected to the control network, will empower the attacker with resources to launch more easily an attack to the controller, for instance." "For instance, by spoofing the address of the network controller, the attacker(using a fake controller) could take over the control of the entire network. A smart attack could persis for only a few seconds,i.e., just the time needed to install special rules on all forwarding devices for its malicious purposes(e.g. traffic cloning). Such attack could be very hard to detect"

%~\cite{khan2016topology} cited by 191: "Compromised controllers: The controllers can also be distributed and exchange information from time-totime to update their states [53]. The module for such distributed communication among controllers can be exploited by the attacker. For instance, Open daylight controller uses ODL-SDNi app for distributed communication among multiple controllers. The problem arises when one of the controllers is performing maliciously and shares wrong information among the controllers. To identify the malicious controller among a pool of controllers is a challenging task due to isolated functionality of each controller. A malicious controller disseminates incorrect topological updates to another controller to make the network malfunction"

%~\cite{maleh2023comprehensive} cited by 44:Another possibility is that the attacker successfully registers a non-legitimate controller at the control level of the SDN network. Using this malware controller, the attacker can influence the availability of other controllers, change the rules, and effectively disable/manipulate the operation of add-ons at the add-on level.

==> tables/related_features.tex <==




\begin{table*}[t]
\caption{\projname{} Features and Evading Existing Detection Mechanism}
%\vspace{-0.8\baselineskip}
%\footnotesize
\label{table:features}
\renewcommand{\arraystretch}{1.5}
\centering
\begin{tabular}{p{4.1cm}p{3.7cm}p{9cm}}
    \toprule
    \textbf{Feature} & \textbf{Related Defense} & \textbf{Evading Detection Mechanism}\\
    \midrule
    Fabricates links without spoofing, hiding, or fabricating packets &\defense{5} TopoGuard(+), \defense{7} Monitoring-based Detection & \defense{5} detects fabricated packets, and \defense{7} identifies spoofing and hiding behaviors. \textbf{\projname{} does not engage in any such activities. }\\
    \midrule
    Explore the vulnerability that flow entries can manipulate link discovery precisely &\defense{7} Monitoring-based Detection & \defense{7} analyzes control plane events  to identify suspicious behaviors but overlooks \textbf{the vulnerability explored by \projname{} that flow entries meant for traffic routing can manipulate link discovery.}\\
    \midrule
    Originates at malicious controller/application  & \defense{1} SPV, \defense{3} Sphinx& \textbf{\projname{} is initiated from control plane} that is trusted by \defense{1}\defense{3} to detect anomalies initiated from data plane.\\
    \midrule
    Utilizes flow entries matching MAC address (with in-port) with higher priority to bypass table-miss/LLDP flow entries &\defense{9} Flow Rule Checker  &\defense{9} examines flow entry conflict with existing flow entries that route data plane traffic.  
    However, 
    %\textbf{\projname{} does not send such flow entries but the ones matching MAC address (with in-port) to override the overlooked table-miss/LLDP flow entries.}
    \update{\defense{9} fails to detect \projname{} because \textbf{the poisonous flow entries by \projname{} conflict with table-miss/LLDP flow entries, which are not monitored by \defense{9}.}}
    \\
    \midrule
    Proactively poisons topology with stealthy flow entries & \defense{8} Voting-based Defense & \textbf{\projname{} leaves benign controllers in \defense{8} to incorrectly process reactive forwarding independently} due to altered topology.\\
    \bottomrule
    
    
    
    Instructs switches to relay link discovery packets  & \defense{2} Latency-based Detection & \update{\defense{2} 
    %is ineffective against \textbf{switch-based relay that \projname{} adopts} due to sufficiently low transmission latency by switches~\cite{al2022link}.\\
    has a high rate of misjudgment, which may fail to detect the \textbf{low-latency switch-based relay of \projname{}} very often~\cite{al2022link,gao2022defense}.}\\
    \hline
    
    Maintains the same degree sequence and high graph similarity &\defense{4} Port-based Detection, \defense{5} TopoGuard(+) & \textbf{Preserved degree sequence by \projname{}} ensures each active port connects to only one link, making \defense{4}\defense{5} ineffective in detection.\\
    
    \hline
    Any controller in cluster discovers deceptive topology independently & \defense{6} Dynamic Cluster & \textbf{\projname{} allows any dynamically assigned leader controllers in \defense{6} to consistently discover the same deceptive topology.} \\
    \hline
\end{tabular}
\vspace{-0.8\baselineskip}
\end{table*}

%~\cite{kreutz2014software}Cited by 6209: " A compromised critical computer, directly connected to the control network, will empower the attacker with resources to launch more easily an attack to the controller, for instance." "For instance, by spoofing the address of the network controller, the attacker(using a fake controller) could take over the control of the entire network. A smart attack could persis for only a few seconds,i.e., just the time needed to install special rules on all forwarding devices for its malicious purposes(e.g. traffic cloning). Such attack could be very hard to detect"

%~\cite{khan2016topology} cited by 191: "Compromised controllers: The controllers can also be distributed and exchange information from time-totime to update their states [53]. The module for such distributed communication among controllers can be exploited by the attacker. For instance, Open daylight controller uses ODL-SDNi app for distributed communication among multiple controllers. The problem arises when one of the controllers is performing maliciously and shares wrong information among the controllers. To identify the malicious controller among a pool of controllers is a challenging task due to isolated functionality of each controller. A malicious controller disseminates incorrect topological updates to another controller to make the network malfunction"

%~\cite{maleh2023comprehensive} cited by 44:Another possibility is that the attacker successfully registers a non-legitimate controller at the control level of the SDN network. Using this malware controller, the attacker can influence the availability of other controllers, change the rules, and effectively disable/manipulate the operation of add-ons at the add-on level.

==> tables/related_threats_backup.tex <==
\begin{table*}
\begin{tabular}{|p{1.5cm}|p{3.5cm}|p{1.3cm}|p{4.5cm}|p{2.5cm}|p{2cm}|}
    \hline
    \textbf{Attack Surface} & \textbf{Attack Methodology}  &
    \textbf{Impact} & \multicolumn{3}{p{7cm}|}{\textbf{Defense}} \\
    \hline
    
     \multirow{5}{1.3cm}{Malicious Host(s)/ Switch}  & \multirow{5}{3.6cm}{\attack{1} 
     Fabricate link A1 -> B2 on controller's view. \\
     Methods: 
     Relay LLDP packet from A1\tablefootnote{Switch A Port 1} to B2 by: 
     \begin{enumerate}[leftmargin=1.4em]
         \item malicious hosts~\cite{hong2015poisoning,skowyra2018effective}
         \item malicious switch~\cite{alimohammadifar2018stealthy} (with "Match: ether-type: 0x88cc, inport:1 Action: output: 2"~\cite{al2022link})
     \end{enumerate}
     Fabricate LLDP packet with "source: A1" and send it to B2 by:
     \begin{enumerate}[leftmargin=1.4em]
        \setcounter{enumi}{2}
         \item malicious hosts~\cite{hong2015poisoning,skowyra2018effective}
         \item malicious switch~\cite{baidya2020link}
     \end{enumerate}}
      & \multirow{5}{1.3cm}{Localized Persistent}
      & \multicolumn{3}{p{10cm}|}{\defense{1} SPV: With benign controller assumption, it sends a probe through the target link. If the link is fabricated, the probe forwarding through A1 will be dropped or fed back to the controller by a switch port other than B2~\cite{alimohammadifar2018stealthy}.}\\
      \cline{4-6}
      & &  & \multicolumn{3}{p{10cm}|}{\defense{2} Latency-based Detection: A link is considered fabricated if its latency is greater than a threshold value~\cite{smyth2017detecting,huang2020towards,al2022link}.}\\
      \cline{4-6}
      & &  & \multicolumn{3}{p{10cm}|}{\defense{3} Sphinx: With benign controller assumption, it builds the flow graph incrementally from Flow-mod OF-message, comparing it with actual flow routings using switch metadata. If a discrepancy is found, fabricating links are on the differing points~\cite{dhawan2015sphinx}.}\\
      \cline{4-6}
      & &  & \multicolumn{3}{p{10cm}|}{\defense{4} Port-based Detection: If an active port connects more than one link, either switch-host link or switch-switch link, one of the switch-switch links is fabricated~\cite{baidya2020link}.}
     \\
     \cline{4-6}
     & &  & \multicolumn{3}{p{10cm}|}{\defense{5} TopoGuard(+): If an active port connects with both host and switch, the link connects switch is fabricated; Authenticating LLDP packets to prevent LLDP packet fabrication~\cite{hong2015poisoning,skowyra2018effective}.} \\
    \cline{1-6}
    
    \multirow{3}{1.6cm}{Malicious Application/ Controller in Cluster} &  \multirow{2}{3.5cm}{\attack{2} Malicious controller shares wrong (topology) information in the controller cluster to cause topology poisoning~\cite{khan2016topology, ropke2018preventing, maleh2023comprehensive}.} & Globalized Ephemeral & \defense{6} Dynamic Cluster: Leader controller is dynamically assigned~\cite{hu2018multi,zhang2018survey,tootoonchian2010hyperflow} and it periodically (e.g., every 100 milliseconds ~\cite{wazirali2021sdn})
    re-discovers the topology from the network independently~\cite{wazirali2021sdn,azzouni2017softdp,dhawan2015sphinx}. & \multirow{2}{2.6cm}{\defense{7} Monitoring-based Defense: Defenses~\cite{habib2022mitigating,zhou2018sdn,ujcich2018cross,ropke2018preventing} audit the controller's or applications' behavior to detect anomalies with backup controller, information flow model or comparison with real network state.}& \multirow{2}{2.3cm}{\defense{8} Voting-based Defense: Fleet~\cite{matsumoto2014fleet},  \textsc{topotrust}~\cite{adjou2022topotrust}, and Mcad-SA\cite{qi2016intensive} depend on the majority to vote out a malicious controller based on odd behaviors around reactive forwarding or spoofing. }\\
    
    \cline{2-4}
    & \multirow{3}{3.6cm}{\attack{3} Insert flow entries to conflict with existing traffic-routing flow entries to detriment flow routings, network policy, or other applications~\cite{khurshid2012veriflow, al2010flowchecker,kazemian2013real, ujcich2018cross}.}& Globalized Persistent & \defense{9} Flow-based Defense: Veriflow~\cite{khurshid2012veriflow}, FlowChecker~\cite{al2010flowchecker}, Netplumber~\cite{kazemian2013real}, and ~\cite{porras2012security} build the flow graph/detection logic with src/dst IPs/ports of flow entries to detect flow rule conflicts and policy violations. & &\\
    \cline{4-6}
    
   % & & & \multicolumn{4}{p{8cm}|}{SDN-RDCD~\cite{zhou2018sdn}, Eirene~\cite{habib2022mitigating} and ProvSDN~\cite{ujcich2018cross} audit the controller's or applications' behavior to detect anomalies with backup controller or information flow model .}\\
   % \cline{4-7}
   % & & & \multicolumn{4}{p{8cm}|}{}\\
    
    \cline{2-6} 
    & \textbf{\projname{}}: Insert stealthy but normal flow entries to poison the topology while maintaining the same degree sequence and high similarity with real topology. It cannot be detected without knowing the switch port MAC addresses and realizing flow entries matching those MAC addresses can influence topology discovery. & Globalized Persistent & \multicolumn{3}{p{10cm}|}{\textbf{No existing defense against \projname{}}.
    Reasons: 
    \projname{} 
    \begin{enumerate}[leftmargin=1.4em]
        \item does not spoof, hide, or fabricate packet (invalidate \defense{5}\defense{7})
        \item maintains same degree sequence (1 port-1 link) (invalidate \defense{4}\defense{5})
        \item originates at malicious controller/application (invalidate \defense{1}\defense{3})
        \item instructs switch (high-speed forwarding) to relay (invalidate \defense{2})
        \item utilizes stealthy flow entries to bypass non-"src/dst IP" table-miss/LLDP flow entries with higher priority(invalidate \defense{9})
        \item proactively poisons topology at one time with stealthy flow entries, letting any benign controller discover the deceptive topology independently and persistently to process reactive forwarding wrongly by themselves. (invalidate \defense{6}\defense{8})
    \end{enumerate}} \\
    \hline
\end{tabular}
\caption{Related Threat and State-of-the-art Defences}\label{table:related_threat}
\end{table*}






%~\cite{kreutz2014software}Cited by 6209: " A compromised critical computer, directly connected to the control network, will empower the attacker with resources to launch more easily an attack to the controller, for instance." "For instance, by spoofing the address of the network controller, the attacker(using a fake controller) could take over the control of the entire network. A smart attack could persis for only a few seconds,i.e., just the time needed to install special rules on all forwarding devices for its malicious purposes(e.g. traffic cloning). Such attack could be very hard to detect"

%~\cite{khan2016topology} cited by 191: "Compromised controllers: The controllers can also be distributed and exchange information from time-totime to update their states [53]. The module for such distributed communication among controllers can be exploited by the attacker. For instance, Open daylight controller uses ODL-SDNi app for distributed communication among multiple controllers. The problem arises when one of the controllers is performing maliciously and shares wrong information among the controllers. To identify the malicious controller among a pool of controllers is a challenging task due to isolated functionality of each controller. A malicious controller disseminates incorrect topological updates to another controller to make the network malfunction"

%~\cite{maleh2023comprehensive} cited by 44:Another possibility is that the attacker successfully registers a non-legitimate controller at the control level of the SDN network. Using this malware controller, the attacker can influence the availability of other controllers, change the rules, and effectively disable/manipulate the operation of add-ons at the add-on level.
